Willingness to Pay for an Electricity Connection: A Choice Experiment Among Rural Households and Enterprises in Nigeria

Rural electrification initiatives worldwide frequently encounter financial planning challenges due to a lack of reliable market insights. This research delves into the preferences and marginal willingness to pay (mWTP) for upfront electricity connections in rural and peri-urban areas of Nigeria. We investigate discrete choice experiment data gathered from 3,599 households and 1,122 Small to Medium-sized Enterprises (SMEs) across three geopolitical zones of Nigeria, collected during the 2021 PeopleSuN project survey phase. Employing conditional logit modeling, we analyze this data to explore preferences and marginal willingness to pay for electricity connection. Our findings show that households prioritize nighttime electricity access, while SMEs place a higher value on daytime electricity. When comparing improvements in electricity capacity to medium or high-capacity, SMEs exhibit a sharp increase in willingness to pay for high-capacity, while households value the two options more evenly. Preferences for the electricity source vary among SMEs, but households display a reluctance towards diesel generators and a preference for the grid or solar solutions. Moreover, households with older heads express greater aversion to connection fees, and male-headed households show a stronger preference for nighttime electricity compared to their female-headed counterparts. The outcomes of this study yield pivotal insights to tailor electrification strategies for rural Nigeria, emphasizing the importance of considering the diverse preferences of households and SMEs.

==> tables/old_hh_mnl_results.tex <==
% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Wed, Aug 16, 2023 - 13:24:40
\begin{tabular}{@{\extracolsep{5pt}}lcccc} 
\\[-1.8ex]\hline 
\hline %\\[-1.8ex] 
% & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
%\cline{2-5} 
%\\[-1.8ex] & \multicolumn{4}{c}{ch} \\ 
\\[-1.8ex] Coefficient & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 fee & $-$0.038$^{***}$ & $-$0.042$^{***}$ & $-$0.042$^{***}$ & $-$0.042$^{***}$ \\ 
  & (0.001) & (0.001) & (0.001) & (0.001) \\ 
  & & & & \\ 
 am & 0.064$^{***}$ & 0.072$^{***}$ & 0.072$^{***}$ & 0.072$^{***}$ \\ 
  & (0.007) & (0.007) & (0.007) & (0.007) \\ 
  & & & & \\ 
 pm & 0.076$^{***}$ & 0.085$^{***}$ & 0.086$^{***}$ & 0.086$^{***}$ \\ 
  & (0.007) & (0.007) & (0.007) & (0.007) \\ 
  & & & & \\ 
 cap\_mid &  & 0.651$^{***}$ & 0.654$^{***}$ & 0.653$^{***}$ \\ 
  &  & (0.058) & (0.058) & (0.058) \\ 
  & & & & \\ 
 cap\_high &  & 1.336$^{***}$ & 1.338$^{***}$ & 1.336$^{***}$ \\ 
  &  & (0.062) & (0.062) & (0.062) \\ 
  & & & & \\ 
 src\_shs &  &  & 0.193$^{***}$ & 0.192$^{***}$ \\ 
  &  &  & (0.065) & (0.065) \\ 
  & & & & \\ 
 src\_smg &  &  & 0.195$^{***}$ & 0.197$^{***}$ \\ 
  &  &  & (0.066) & (0.066) \\ 
  & & & & \\ 
 src\_grid &  &  & 0.153$^{**}$ & 0.156$^{**}$ \\ 
  &  &  & (0.065) & (0.065) \\ 
  & & & & \\ 
 crr\_prv &  &  &  & 0.098 \\ 
  &  &  &  & (0.057) \\ 
  & & & & \\ 
 crr\_com &  &  &  & 0.083 \\ 
  &  &  &  & (0.056) \\ 
  & & & & \\ 
\hline \\[-1.8ex] 
Observations & 7,090 & 7,090 & 7,090 & 7,090 \\ 
Log Likelihood & $-$3,168.857 & $-$2,906.090 & $-$2,900.166 & $-$2,898.433 \\ 
$\rho^2$ & 0.3551 & 0.4086 & 0.4098 & 0.410141\\ 
AIC & 6343.71 & 5822.18 & 5816.33 & 5816.87 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

==> tables/socioeconomic_terms.tex <==

\begin{table}
    \centering
    \begin{tabular}{cc}
         Factor& Question in PeopleSuN survey\\
         Weekly expenditure per member& \\
         Age of household head& \\
         Married household head& \\
         Male household head& \\
         Female need permission buying clothes& \\
 Household size&\\
 Take loan(s) before&\\
 Trust in government&\\
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

==> tables/zone_mnl_results.tex <==
% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Wed, Aug 16, 2023 - 13:24:40
\begin{tabular}{@{\extracolsep{5pt}}lcccc} 
\\[-1.8ex]\hline 
\hline %\\[-1.8ex] 
% & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
%\cline{2-5} 
%\\[-1.8ex] & \multicolumn{4}{c}{ch} \\ 
\\[-1.8ex] Coefficient & North Central & South South & North West & All\\ 
\hline \\[-1.8ex] 
 fee & $-$0.050$^{***}$ & $-$0.036$^{***}$ & $-$0.046$^{***}$ & $-$0.042$^{***}$ \\ 
  & (0.002) & (0.002) & (0.002) & (0.001) \\ 
  & & & & \\ 
 am & 0.105$^{***}$ & 0.067$^{***}$ & 0.057$^{***}$ & 0.072$^{***}$ \\ 
  & (0.013) & (0.012) & (0.012) & (0.007) \\ 
  & & & & \\ 
 pm & 0.123$^{***}$ & 0.067$^{***}$ & 0.080$^{***}$ & 0.086$^{***}$ \\ 
  & (0.013) & (0.012) & (0.013) & (0.007) \\ 
  & & & & \\ 
 cap\_mid & 0.265$^{**}$ & 1.029$^{***}$ & 0.654$^{***}$ & 0.653$^{***}$ \\ 
  & (0.106) & (0.101) & (0.102) & (0.058) \\ 
  & & & & \\ 
 cap\_high & 0.727$^{***}$ & 1.923$^{***}$ & 1.353$^{***}$ & 1.336$^{***}$ \\ 
  & (0.108) & (0.113) & (0.111) & (0.062) \\ 
  & & & & \\ 
 srca solar home system & 0.305$^{**}$ & 0.080 & 0.277$^{**}$ & 0.192$^{***}$ \\ 
  & (0.120) & (0.110) & (0.116) & (0.065) \\ 
  & & & & \\ 
 srca solar microgrid & 0.106 & 0.190$^{*}$ & 0.324$^{***}$ & 0.197$^{***}$ \\ 
  & (0.124) & (0.110) & (0.115) & (0.066) \\ 
  & & & & \\ 
 srcthe grid & 0.141 & 0.155 & 0.186 & 0.156$^{**}$ \\ 
  & (0.122) & (0.109) & (0.114) & (0.065) \\ 
  & & & & \\ 
 crra private power company & $-$0.112 & 0.096 & 0.037 & 0.014 \\ 
  & (0.106) & (0.095) & (0.100) & (0.057) \\ 
  & & & & \\ 
 crrthe state electricity company & $-$0.200$^{*}$ & 0.026 & $-$0.121 & $-$0.083 \\ 
  & (0.106) & (0.094) & (0.099) & (0.056) \\ 
  & & & & \\ 
\hline \\[-1.8ex] 
Observations & 2,368 & 2,359 & 2,363 & 7,090 \\ 
Log Likelihood & $-$868.091 & $-$1,013.314 & $-$934.554 & $-$2,898.433 \\ 
$\rho^2$ & 0.3551 & 0.4086 & 0.4098 & 0.410141\\ 
AIC & 6343.71 & 5822.18 & 5816.33 & 5816.87 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
